A positivity-preserving and conservative high-order flux reconstruction method for the polyatomic Boltzmann--BGK equation

In this work, we present a positivity-preserving high-order flux reconstruction method for the polyatomic Boltzmann--BGK equation augmented with a discrete velocity model that ensures the scheme is discretely conservative. Through modeling the internal degrees of freedom, the approach is further extended to polyatomic molecules and can encompass arbitrary constitutive laws. The approach is validated on a series of large-scale complex numerical experiments, ranging from shock-dominated flows computed on unstructured grids to direct numerical simulation of three-dimensional compressible turbulent flows, the latter of which is the first instance of such a flow computed by directly solving the Boltzmann equation. The results show the ability of the scheme to directly resolve shock structures without any ad hoc numerical shock capturing method and correctly approximate turbulent flow phenomena in a consistent manner with the hydrodynamic equations.

==> analysis.tex <==
 %!TEX root = ./main.tex
\section{Analysis}
\label{sec:analysis}

==> notes.tex <==
%!TEX root = ./main.tex
\section{Notes}\label{sec:notes}
TODO
\begin{itemize}
    \item Make plugins work with distributions
    \item Shock capturing
    \item Boundary conditions
    \item Estimating max bounds from speed of sound
\end{itemize}




\begin{equation}
    \partial_t f (\mathbf{x}, \mathbf{u}, t) + \mathbf{u} {\cdot} \nabla f = \frac{g(\mathbf{u}, t) - f}{\tau}
\end{equation}

\begin{equation}
    \int_{\mathbb R^d}f \boldsymbol{\psi}\ \mathrm{d}\mathbf{u} = [\rho, \rho \mathbf{U}, \rho E]^T
\end{equation}
\begin{equation}
    \psi = [1, \mathbf{u}, \frac{1}{2} (\mathbf{u}{\cdot}\mathbf{u})]
\end{equation}

\begin{equation}
    f_0(u) = g(u) = M(u) = \rho (\lambda/\pi)^{d/2} \exp(-\lambda(u - U)^2)
\end{equation}

\begin{equation}
    \lambda = \frac{1}{2}\frac{\rho}{e}, \quad \quad e = p/(\gamma -1)
\end{equation}

\begin{equation}
    \Delta t \sim \mathcal O (CFL*h/\max(v))
\end{equation}


$\gamma = 3$ for a 1D/1V system, $\gamma = 5/3$ for 2D/2V, and $\gamma = 7/5$ for 3D/3V.

\subsection{Equilibrium distribution}

Equilibrium state minimizes the entropy function $f \log f$, i.e.,
\begin{equation}
    g(u) = \underset{x > 0}{\arg \min} \int_{-\infty}^{\infty} x(u) \log x(u) \ \mathrm{d}u
\end{equation}
Analytically, it's the Maxwellian
\begin{equation}
    g(u) = M(u) = A \exp (-B(u - C)^2) = \rho (\lambda/\pi)^{d/2} \exp(-\lambda(u - U)^2)
\end{equation}
but the relation 
\begin{equation}
    \int_{-\infty}^{\infty} g \psi\ \mathrm{d}u = [\rho, \rho U, \rho E]
\end{equation}
doesn't hold discretely.

Let 
\begin{equation}
    \mathbf{M}{\cdot}\mathbf{x} \approx \int_{-\infty}^{\infty} x \ \mathrm{d}u
\end{equation}
and 
\begin{equation}
    \mathbf{M}{\cdot} \left(\boldsymbol{\psi}_j \odot \mathbf{x}) \right) \approx \int_{-\infty}^{\infty} x \psi_j\ \mathrm{d}u \ \forall \ j \in \{1, ..., d+2 \}
\end{equation}

Discrete conditions for equilibrium state
\begin{equation}
    \mathbf{f} = \underset{g > 0}{\arg \min}\left [ \mathbf{M}{\cdot}(\mathbf{g} \log \mathbf{g}) \right] s.t.\ \mathbf{g}_i > 0 \ \forall i \ \ and\ \mathbf{M}{\cdot} \left(\boldsymbol{\psi}_j \odot \mathbf{g}) \right) = \mathbf{U}_j \ \forall \ j
\end{equation}
Let
\begin{equation}
    \boldsymbol{\alpha} = [A', B', C']
\end{equation}
The solution takes on an exponential form with modified coefficients $A', B', C'$
\begin{equation}
    \mathbf{f} = A' \exp (-B'(\mathbf{u} - C')^2) = \mathbf{f}(\boldsymbol{\alpha})
\end{equation}
Solve the root-finding problem
\begin{equation}
    \mathbf{F}(\boldsymbol{\alpha}) = \mathbf{0}, \quad \quad \mathbf{F}(\boldsymbol{\alpha}) = \mathbf{M}{\cdot} \left(\boldsymbol{\psi} \odot \mathbf{f}) \right) - U
\end{equation}
using the Jacobian
\begin{equation}
    \mathbf{J}_{i,j}(\mathbf{\alpha}) = \mathbf{M}{\cdot} \left(\boldsymbol Z_i \odot \boldsymbol{\psi}_j \odot \mathbf{f}(\mathbf{\alpha})) \right)
\end{equation}
where
\begin{equation}
    \boldsymbol{Z} = [1/A, -(u - C)^2, 2B(u-C)]
\end{equation}

% In the limit of vanishing Knudsen number, the NS equations are recovered with $\nu = \tau 2 \lambda$


% $\lambda = m/(2kT)$

% From NS:

% $\gamma/c_p e = T$ where $e = (E - KE)/\rho$

% From paper: $Kn = \ell/L_0$ where $\ell$ is the mean free path and $L_0$ is the reference length scale. This is related to the relaxation time $\tau$ by the relation \begin{equation}
%     \tau = \frac{4 \ell}{\pi C}
% \end{equation}
% where $C$ is the most probable particle velocity. 

From wiki:
\begin{equation}
    Kn = \sqrt{\frac{\gamma \pi}{2}} Ma/Re = \sqrt{\frac{\gamma \pi}{2}} \frac{\mu}{\rho L_0 c_s}, \mathrm{where} \  c_s = \sqrt{\frac{\gamma R T}{M}} = \sqrt{\frac{\gamma k_B T}{m}} = \sqrt{\frac{\gamma P}{\rho}}
\end{equation}

From Orszag:
\begin{equation}
    \nu = \tau \theta -> \mu = \rho\tau \theta
\end{equation}
where
\begin{equation}
    \theta = P/\rho
\end{equation}

so we get
\begin{equation}
    Kn = \sqrt{\frac{\gamma \pi}{2}} \frac{\tau P}{\rho L_0 c_s} = \sqrt{\frac{\gamma \pi}{2}} \frac{\tau}{L_0} \frac{P}{\rho} \sqrt{\frac{\rho}{\gamma P}} = \sqrt{\frac{\gamma \pi}{2}} \frac{\tau}{L_0} \frac{c_s}{\gamma} = \frac{\lambda}{L_0}
\end{equation}

Shock thickness:
\begin{equation}
    L = \frac{\max | \partial_x \rho |}{| \rho_2 - \rho_1|}
\end{equation}

Inverse thickness ratio:
\begin{equation}
    \lambda/L 
\end{equation}
where
\begin{equation}
    \lambda = \sqrt{\frac{\gamma \pi}{2}} \tau \frac{c_s}{\gamma} = 
\end{equation}

% From NASA
% \begin{equation}
%     c_p = c_v + R
% \end{equation}
% \begin{equation}
%     \gamma = c_p/c_v
% \end{equation}
% \begin{equation}
%     R/c_v = (c_p - c_v)/c_v = (\gamma - 1)
% \end{equation}
% \begin{equation}
%     R/c_p = (\gamma - 1)/\gamma
% \end{equation}
Noticing that if setting $\zeta$ too low (not enough velocity space range), then weird behavior happens on Sod and other test cases near the boundaries (gaining pressure etc.)
